MR.Rec: Synergizing Memory and Reasoning for Personalized Recommendation Assistant with LLMs

The application of Large Language Models (LLMs) in recommender systems faces key challenges in delivering deep personalization and intelligent reasoning, especially for interactive scenarios. Current methods are often constrained by limited context windows and single-turn reasoning, hindering their ability to capture dynamic user preferences and proactively reason over recommendation contexts. To address these limitations, we propose MR.Rec, a novel framework that synergizes memory and reasoning for LLM-based recommendations. To achieve personalization, we develop a comprehensive Retrieval-Augmented Generation (RAG) system that efficiently indexes and retrieves relevant external memory to enhance LLM personalization capabilities. Furthermore, to enable the synergy between memory and reasoning, our RAG system goes beyond conventional query-based retrieval by integrating reasoning enhanced memory retrieval. Finally, we design a reinforcement learning framework that trains the LLM to autonomously learn effective strategies for both memory utilization and reasoning refinement. By combining dynamic memory retrieval with adaptive reasoning, this approach ensures more accurate, context-aware, and highly personalized recommendations. Extensive experiments demonstrate that MR.Rec significantly outperforms state-of-the-art baselines across multiple metrics, validating its efficacy in delivering intelligent and personalized recommendations. We will release code and data upon paper notification.

==> Tables/memory_construction_efficiency.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet4'
\begin{table}[t]
  \centering
  \caption{Statistics and costs of the local memory and global memory mechanisms in our \ourmodel framework.}
  \vspace{-0.12in}
  \small
  \setlength{\tabcolsep}{2.2mm}
  {
    \begin{tabular}{lcc}
    \toprule
        & \multicolumn{1}{c}{\textbf{Local Memory}} & \multicolumn{1}{c}{\textbf{Global Memory}} \\
    \midrule
    Source Users & 3,000      & 157 \\
    Input Tokens (M) &   385.21    & 0.48 \\
    Output Tokens (M) &   42.00    & 0.06 \\
    Memory Entries &  73,078     & 1,970 \\
    \midrule
    Total Time (s)  &   2,435    & 121 \\
    Per-entry Time (s) & 0.07   & 0.06 \\
    API Cost (GPT-4o-mini) &   54.09    &  0.07 \\
    Per-entry Cost &    $7.4 \times 10^{-4}$   & $3.6 \times 10^{-5}$ \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:memory_construction_efficiency}%
  \vspace{-0.2in}
\end{table}%


==> Tables/memory_token_efficiency.tex <==
% Table generated by Excel2LaTeX from sheet 'data statistics'
\begin{table}[htbp]
  \centering
  \caption{Comparison of token efficiency between our \ourmodel and baselines. }
   \resizebox{0.49\textwidth}{!}{
    \begin{tabular}{cccc}
    \toprule
    Memory Setting & \makecell[c]{ Avg. Memory\\Tokens} & {\makecell[c]{R@100\\(GPT-4o)}} & \makecell[c]{Efficiency\\(R@100/100 tokens)} \\
    \midrule
    \makecell[c]{Recent 10 interactions} & 283.51 & 0.261 & 0.092 \\
    \makecell[c]{Static user profile} & 492.7 & 0.261 & 0.053 \\
    MR.Rec & 95.43 & 0.285 & 0.299 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:memory_token}%
\end{table}%

